Universal Average-Case Optimality of Polyak Momentum

Polyak momentum (PM), also known as the heavy-ball method, is a widely used optimization method that enjoys an asymptotic optimal worst-case complexity on quadratic objectives. However, its remarkable empirical success is not fully explained by this optimality, as the worst-case analysis -- contrary to the average-case -- is not representative of the expected complexity of an algorithm. In this work we establish a novel link between PM and the average-case analysis. Our main contribution is to prove that any optimal average-case method converges in the number of iterations to PM, under mild assumptions. This brings a new perspective on this classical method, showing that PM is asymptotically both worst-case and average-case optimal.

==> proofs/optimal_fisher_proof.tex <==
\begin{proof} 
    consider any polynomial $P=P_t$ of degree $t$ such that $P(0) = 1$. Now, consider the residual polynomial $R$ where
    \[
        P(x)-P^*(x) = xR(x), \quad \deg(R) = t-1.
    \]
    The residual polynomial is multiplied by $\xx$ since $0$ is a root of $P(x)-P^{\star}(x)$, since
    \[
        P(0)-P^{\star}(0) = 1-1 = 0.
    \] 
    We now show that if 
    \[
        P^{\star} \text{ is orthogonal w.r.t } \lambda\mu(\lambda) \qquad \text{and} \qquad  P \in \arg\min_P \langle P, P \rangle = \int_{\mathbb
        R}P^2(\lambda)\lambda\mu(\dif \lambda),
    \]
    then $R = 0$, thus implying that $P^{\star} = P$. Indeed,
    \[
        \langle P,P \rangle = \langle P^{\star}, P^{\star} \rangle + \langle \xx R, \xx R \rangle + 2 \langle P^{\star}, \xx R \rangle
    \]
    However,
    \begin{align*}
         \langle P^{\star}, \xx R \rangle & = \int  P^{\star}(\lambda) \lambda R(\lambda) \dif \mu(\lambda)\\
         & = \int  P^{\star}(\lambda)  R(\lambda) \lambda\dif \mu(\lambda)\\
         & = 0
    \end{align*}
    The last equality follows from the fact that the degree of $P^{\star}$ is equal to $t$. This means the polynomial is orthogonal to all other polynomial of degree $t-1$, w.r.t to $\lambda\dif \mu(\lambda)$. Thus,
    \[
        \langle P,P \rangle = \langle P^*, P^* \rangle + \langle \xx R, \xx R \rangle = \underbrace{\|P^{\star}\|^2}_{>0} + \underbrace{\|\xx R\|^2}_{\geq 0}.
    \]
    Since $P$ is the minimal polynomial, $R$ has to be always $0$, which proves the proposition.
\end{proof}

==> proofs/optimal_polynomial.tex <==
\begin{proof}
    We start with the definition of the algorithm, then we show that it actually builds the optimal polynomial \eqref{eq:optimal_polynomial}. Indeed, by removing $\xx^{\star}$ on both sides,
    \[
        \xx_{t}-\xx^{\star} = a_t(\xx_{t-1}-\xx^{\star}) - (1-a_t)(\xx_{t-2}-\xx^*) - b_t \nabla f(\xx_{t-1})
    \]
    By definition of our quadratic function, its gradient reads
    \[
        \nabla f(\xx_{t-1}) = \HH(\xx_{t-1}-\xx^{\star}).
    \]
    All together, the recursion becomes
    \[
        \xx_{t}-\xx^{\star} = a_t(\xx_{t-1}-\xx^{\star}) - (1-a_t)(\xx_{t-2}-\xx^{\star}) - b_t \HH(\xx_{t-1}-\xx^{\star})
    \]
    However, we have that $\xx_0-\xx^{\star}$ and $\xx_1-\xx^{\star}$ are polynomials, since
    \begin{align*}
        \xx_0-\xx^{\star} & = \HH^0(\xx_0-\xx^{\star}) = p_0^{\star}(\HH)(x_0-x^{\star})\\
        \xx_1-\xx^{\star} & = x_0-x^{\star} - b_1 \HH^0(\xx_0-\xx^{\star}) = p_1^{\star}(\HH)(\xx_0-\xx^{\star}).
    \end{align*}
    Using this argument recursively, we have that
    \[
        \xx_{t}-\xx^{\star} = \left(a_tP_{t-1}^{\star}(\HH) - (1-a_t)P_{t-2}^{\star}(\HH) - b_tP_{t-1}^{\star}(\HH)\right)(\xx_0-\xx^{\star}) = P_t^{\star}(\HH)(x_0-x^*).
    \]
    Since, by construction, $p^{\star}$ is the solution of \eqref{eq:optimal_polynomial}, the algorithm is optimal. We now show that the square in the integral can be simplified. Without any loss of generality we consider $\beta = 0$. Indeed,
    \[
        \int_{\mathbb{R}^+} P_t^2(\lambda) \mu(\lambda)\dif\lambda = \int_{\mathbb{R}^+} P_t(\lambda) \left( \lambda \frac{P_t(\lambda)-P_t(0)}{\lambda} + P_t(0) \right) \mu(\lambda)\dif\lambda.
    \]
    Let $Q(\lambda) = \frac{P_t(\lambda)-P_t(0)}{\lambda}$. This is a polynomial of degree $t-1$ since we took $P_t$, then we removed the independent term, then divided by $\lambda$. Since the sequence $\{P_i\}$ forms a basis of polynomial, we have that $P_t$ is orthogonal to all polynomials of degree less than $t$ w.r.t. $\lambda \mu(\lambda)$. In this case, $P_t$ is orthogonal to $Q$, thus
    \[
        \int_{\mathbb{R}^+} P_t^2(\lambda) \mu(\lambda)\dif\lambda = \int_{\mathbb{R}^+} P_t(\lambda) Q(\lambda) \lambda \mu(\lambda)\dif\lambda  + \int_{\mathbb{R}^+} P_t(\lambda) P_t(0) \mu(\lambda)\dif\lambda = \int_{\mathbb{R}^+} P_t(\lambda)  \mu(\lambda)\dif\lambda,
    \]
    where the last equality follows from the fact that $P$ is a normalized polynomial, thus $P(0) = 1$.
\end{proof}
